Many-time physics in practice: characterising and controlling non-Markovian quantum stochastic processes

Every year, substantial theoretical and experimental progress is made towards the realisation of a genuinely new computational paradigm in the construction of a quantum computer. But progress is fractal; to make headway is to unearth the next set of obstacles. Decades of work has so far overcome physical, mathematical, engineering, and information theoretic obstacles to produce the remarkable high-fidelity devices we see today. But these devices must be near perfect to be useful. Indeed, advancements so far have precipitated sensitivity to a host of complex dynamical and control-based effects. Chief among these today are non-Markovian memory effects, where interactions between a quantum system and its surrounding environment can give rise to multi-time correlations. In this thesis, we address this issue and formally present a generalisation of quantum process tomography, called process tensor tomography (PTT). This establishes the ability to rigorously and systematically characterise non-Markovian open quantum systems, resolving many long-standing issues in the field. In the first part of this work, we present an original review of the literature and motivate the problem at hand. In the second, we develop the framework of PTT, including experiment design, post-processing algorithms, and both simulated and near-term device demonstrations. In particular, we demonstrate this as a tool for obtaining in-depth diagnostics about the nature and origin of temporal quantum correlations. Lastly, we dedicate our efforts to efficiency and self-consistency. To this effect, we explore theoretically processes with sparse memory structures. We then leverage this to develop various efficient estimation techniques tailored for different settings. The result is a robust and lightweight framework capable of both reconstructing and optimally controlling any non-Markovian open quantum dynamics.

==> Chapters/Chapter09.tex <==
\chapter{Designing informationally complete quantum instruments}
\label{chap:designing-instruments}
\noindent\colorbox{olive!10}{%
	\begin{minipage}{\textwidth} %0.955 seems about in line with underline
		\textcolor{Maroon}{\textbf{Chapter Summary}}\newline
		The usual regime of unitary control is insufficient to determine detailed information about different multi-time correlations. In this Chapter, we resolve this issue by developing a precise scheme to use nearby qubits as probes of a system's multi-time correlations.
		\par\vspace{\fboxsep}
		\colorbox{cyan!10}{%
			\begin{minipage}{\dimexpr\textwidth-2\fboxsep}
				\textcolor{RoyalBlue}{\textbf{Main Results}} 
				\begin{itemize}
					\item By driving interactions with neighbouring qubits, we can use them as a source of non-Markovianity to expand the control space.
					\item We employ a single PTT characterisation to learn the whole space of noisy quantum instruments from an ancilla qubit. In turn, these can then be used on the system to learn its entire process tensor.
				\end{itemize}
		\end{minipage}}
\end{minipage}}
\clearpage

\com{Include a discussion of some condition numbers and maybe a set of different results across devices}

\com{Also include I think the different bootstrapped process tensor experiments}




==> Chapters/Chapter13.tex <==
\chapter{Filtering Crosstalk From Bath non-Markovianity via Spacetime Classical Shadows}
\label{chap:crosstalk-filter}
\noindent\colorbox{olive!10}{%
	\begin{minipage}{\textwidth} %0.955 seems about in line with underline
		\textcolor{Maroon}{\textbf{Chapter Summary}}\newline
		It is a keen priority to understand and eliminate non-Markovian effects in quantum devices. This requires pinpointing the origins of various noise sources. But the problem is obfuscated by the fact that neighbouring qubits can also naturally couple to each other and give rise to similar types of effects, known as crosstalk. Distinguishing the interplay with neighbouring qubits from that of an inaccessible environment is a pertinent question -- can the problems be resolved with more sophisticated control, or should the priority be to address defects in the fabrication process? To solve this problem, we generalise the recent framework of classical shadow tomography. The technique of classical shadows is a method by which properties of quantum states can be extracted with exponentially fewer measurements. We extend this concept to the spatiotemporal domain. This shows how one may learn spacetime quantum correlations in an efficient way, which is a highly useful tool. We showcase how it resolves the above problem. We derive a procedure that filters out the complex effects of crosstalk to reduce to lay bare the complex environment. This causally tests the source of non-Markovian effects -- whether they originate from environment defects or controllable neighbouring qubits, and the geometric location of those defects.

		\par\vspace{\fboxsep}
		\colorbox{cyan!10}{%
			\begin{minipage}{\dimexpr\textwidth-2\fboxsep}
				\textcolor{RoyalBlue}{\textbf{Main Results}}
				\begin{itemize}
					\item We consider the application of classical shadow tomography to multi-time processes on multi-qubit devices, finding that one can naturally filter out passive crosstalk between qubits.
					\item We present a series of numerical results on a lattice of interacting qubits to demonstrate the ability to geometrically local inaccessible non-Markovian defects amid a device.
				\end{itemize}
		\end{minipage}}
\end{minipage}}
\clearpage

\section{Introduction}
\rewrite{
In the race to fault tolerant quantum computing, magnified sensitivity to complex dynamics in open quantum systems requires increasingly tailored characterisation and spectroscopic techniques~\cite{chalermpusitarak2021frame,ferrie2018bayesian,nielsen-gst,PhysRevX.9.021045,White-NM-2020,white2022non,youssry2020characterization,von2020two}. Correlated dynamics are one particularly pernicious class of noise, and can be generated from a variety of sources, including inhomogeneous magnetic fields, coherent bath defects, and nearby qubits, see Figure~\ref{fig:crosstalk_idea}a~\cite{paladino20141,mavadia2018experimental}. Concerningly, these effects are often omitted from typical quantum error correction noise models despite being ubiquitous in noisy intermediate-scale quantum (NISQ) hardware~\cite{Clader2021,White-NM-2020,white2021many, white2022non,correlated-qec,Harper2020}.

Temporal -- or non-Markovian -- correlations are elements of error that are correlated between different points in time, as mediated by interactions with an external system~\cite{Pollock2018a,white2022non}. The specific mediator of these effects is both conceptually and experimentally relevant device information. Is it something we can control, or is it part of the inaccessible bath? Entangling crosstalk, such as the always-on $ZZ$ interactions in transmon qubits~\cite{PhysRevA.101.052308}, can generate temporal correlations. But whether the dynamics look non-Markovian depends on whether it is feasible or not to dilate the characterisation to multiple qubits -- which, typically, it is not. 
Since crosstalk and non-Markovianity can easily be conflated, it is crucial to find robust methods that can not only account for their behaviour, but distinguish them.}
\begin{figure}[h]
	\centering
	\includegraphics[width=0.75\linewidth]{Shadows_Paper/ST_Fig_1.pdf}
	\caption{System of interacting qubits and an inaccessible non-Markovian environment. \textbf{a} A single qubit may interact via crosstalk mechanisms with other qubits in a quantum device, as well as defects in the bath and stochastic classical fields. \textbf{b} The non-Markovian correlations for that system may be separated into different causal pathways by which the correlations are mediated. Causal breaks (depicted in grey) erase any temporal correlations from a given pathway, allowing one to infer the various contributions to total non-Markovianity from nearby qubits and environment.}
	\label{fig:crosstalk_idea}
\end{figure}

In this Chapter, we establish a systematic, concrete, and efficient approach to the two pragmatic questions: (1) if non-Markovian dynamics are detected across different timescales for a qubit, do they come from neighbouring qubits or a nearby bath? And (2) how can we determine when two qubits are coupled to a shared bath generating common cause non-Markovian effects, versus independent sources or direct interaction?
The solutions here have highly practical implications. Namely, whether curbing the correlated effects is achievable through more intricate control of the various subsystem, or whether more careful attention needs to be paid to defects in the fabrication process~\cite{winick2021simulating,wei2022hamiltonian}.
%\com{cite progress in dynamic measurements, say that the procedure is suitable for near-term hardware.}
%One might, for instance, like to characterise the non-Markovian effects solely from higher energy levels in transmon qubits.
Up to this point, attempts to answer the first question have been mostly heuristic: detect non-Markovian behaviour, and then search through candidate explanations of the underlying physics to see whether this explains the phenomena~\cite{tripathi2022suppression,Sarovar2020detectingcrosstalk,krinner2020benchmarking}.
%come back to this. include the above citations and also mckay2020correlated, maybe Harper2020, rudinger2021experimental, hashim2022benchmarking, helsen2021estimating
But this approach is not scalable, and highly model-dependent.
Process tensor tomography (PTT) is a recently developed generalisation to quantum process tomography, and can guarantee an answer to these questions and more, but the number of experiments required grows as $\mathcal{O}(d^{2kn+n})$ to find correlations across $k$ steps over $n$ qudits~\cite{white2022non}. \par

The basic premise of our work is to apply the method of classical shadows to PTT, resolving these problems. Then, instead of reconstructing the whole multi-time process for an entire quantum register, we can simply look at process marginals. 
This gives us access to maximal depolarising channels at no extra cost on the remainder of the qubits at each time. These operations act as causal breaks on controllable systems. When suitably placed, these operations eliminate temporal correlations as mediated on the chosen Hilbert spaces, thus allowing non-Markovian sources to be causally tested. We illustrate this idea in Figure~\ref{fig:crosstalk_idea}b. The end result is the simultaneous determination of the bath-mediated non-Markovianity on all qubits.
%\com{Compute the scaling cost of our method, also compute it for, e.g., only nearest neighbour shared baths or something. Specify}
%We show how these operations constitute a free resource under the regime of classical shaxdows as applied to spatiotemporal correlations in PTT.
Our approach hence only depends on the individual system size (in this work, qubits), and is a physics-independent way for us to test the relevant hypotheses. %The definition of controllable here is also flexible. Although we consider extremal case where all other register qubits are erased, one might aim to probe arbitrary pathways to causally test temporal correlation origins. 
We are also able to simultaneously compute all $\binom{nk}{k}$ spacetime marginals (with resources growing exponentially in $k$), i.e. the generic process correlations between groupings of qubit-time coordinates. This extends the randomised measurement toolkit to the spatiotemporal domain~\cite{elben2022randomized}. Note that while this approach can also be used to characterise crosstalk, extensive work has already been conducted on this topic, and so we do not concentrate on these spatial correlations~\cite{Sarovar2020detectingcrosstalk,rudinger2021experimental, helsen2021estimating}. Instead, we focus on the ability to filter out crosstalk effects and study what is left over from the bath.

%\com{Mention somewhere that the shared bath idea can also just be used to generically study spatiotemporally spreading errors on an arbitrarily-sized lattice}

%The experimental procedure requires a sequences of projective measurements and independent fresh preparations, each in random Pauli bases. The relevant data for spatiotemporal marginals are then computed using the method of classical shadows and the process marginals estimated using maximum likelihood PTT.
%The information generated supplies the non-Markovian temporal correlations as mediated exclusively by an inaccessible bath, as well non-Markovian spatiotemporal correlations mediated by a shared bath between multiple qubits. The correlations can also be scrutinised by the standard quantum information toolkit, identifying for example whether the mediators are classical or quantum. This information can immediately be fed forward into fabrication processes, as well as the error suppression, mitigation and correction part of the software stack.
%Although the focus application in this work is noise triangulation, the techniques developed are pertinent to other forms of environmental determination, such as with multi-qubit quantum sensors. Moreover, this capability extends the randomised measurement toolbox to the spacetime setting~\cite{elben2022randomized}.

% \com{NM correlations can be confused for crosstalk? see Sarovar}
% This work is structured as follows: we begin with a review of process tensor tomography, and introduce applications of classical shadows to determine spacetime correlations. Next, we show how the shadow procedure naturally implements causal breaks which can be used to Markovianise dynamics across controllable spaces. The remaining temporal correlations can thus be attributed to interactions with an inaccessible (classical or quantum) bath.
% We demonstrate numerically this procedure on a lattice of interacting qubits with defects, showing how one may triangulate non-Markovian environmental defects and establish common cause relations between different parts of the register.




\section{Erasing non-Markovian Pathways}
The above procedure suffices to estimate marginals of a process tensor, which we show for completeness in the appendix. In short, we estimate the required observables to uniquely fix the process marginal, and then employ a maximum likelihood algorithm to determine a physically consistent process tensor. This comes equipped with the familiar logarithmic scaling properties of classical shadows in the number of marginals. We consider two possible applications of spatiotemporal classical shadows, and supplement with numerical demonstrations.
\begin{figure}
	\centering
	\includegraphics[width=0.75\linewidth]{Shadows_Paper/ST_Fig_3.pdf}
	\caption{A numerical simulation demonstrating the proposed technique to isolate environmental effects. A grid of 15 qubits is simulated with crosstalk effects and an inaccessible non-Markovian defect. \textbf{a} Determining the non-Markovianity on each qubit individually (with the remainder idle) is not very informative, since each qubit looks non-Markovian due to passive crosstalk. \textbf{b} After learning all of the shadow marginals $\Upsilon_{2:0}^{(q_j)}$, the crosstalk is filtered out to reveal which qubits possess temporal correlations from the environment.}
	\label{fig:simulated-baths}
\end{figure}
\emph{Recovering process marginals.--}

Although collecting shadows suffices to estimate properties of the process marginals, they will not in general be able to reconstruct a physical estimate of the process marginals. To this effect we estimate enough observables to constitute informationally complete information about the process tensor, and then employ maximum-likelihood PTT to process the data and obtain a physical estimate. The advantages of a physical (positive, causal) estimate is that we make use of information theoretic tools that rely on the postitivity of the state. 

The total number of shadows required to estimate $M$ observables $O_i$ to a precision of $\epsilon$ was shown by Huang et al. to be~\cite{huang-shadow}
\begin{equation}
	N_{\text{shots}} = \mathcal{O}\left(\frac{\log M}{\epsilon^2} \max_{1\leq i \leq M}\| O_i\|_{\text{shadow}}\right).
\end{equation}
For an $l$-local Pauli observable, this shadow norm is shown to be $3^l$. The numerical simulations in the main text are two step processes, whose Choi forms are equivalent to a five qubit state. The remainder of the observables on the process are trivial, i.e. $\mathbb{I}$. In the Choi picture, this is equivalent to a maximally depolarising channel. Explicitly,
\begin{equation}
	\mathcal{R}_\lambda[\rho] := (1 - \lambda)\rho + \lambda\mathbb{I}/2,
\end{equation}
then $\hat{\mathcal{R}}_{1} = \mathbb{I}/2$, with normalisation chosen to be $d$.

Causality conditions fix the expectations of $\sum_{j=1}^k(d^2-1)d^{4j-2}$ Pauli operators. For a two step process then, this leaves $M=820$ expectation values to estimate. From the bounds given in Ref.~\cite{huang-shadow}, we therefore have $N_{\text{shots}} = \mathcal{O}(\log(N_{\text{qubits}}\cdot M)/\epsilon^2 3^5)\approx 2\times 10^7$ measurements in the worst case, which is what we use in our numerical experiments. The median-of-means algorithm from Ref.~\cite{huang-shadow} is used to estimate an informationally complete set of observables for each process marginal, and the maximum likelihood estimation obtained using the methods developed in Ref.~\cite{white2022non}.

% An estimate for the map is coupled with metric of goodness (the likelihood) which quantifies how consistent the map is with the data. The cost function is then minimised while enforcing the physicality of the map.
% The stored data vector in PTT is the object $n_{i,\vec{\mu}}$, which contains the observed measurement probabilities for the $i$th effect of an IC-POVM, subject to a sequence of $k$ operations $\bigotimes_{j=0}^{k-1}\mathcal{B}_j^{\mu_j}$. As is typical in MLE tomography, this data is fit to a model for the process, $\Upsilon_{k:0}$, such that
% \begin{equation}
	% \label{PT-vector-est}
	%     p_{i,\vec{\mu}} = \text{Tr}\left[(\Pi_i \otimes  \mathcal{B}_k^{\mu_{k-1}\text{T}}\otimes \cdots \otimes \mathcal{B}_0^{\mu_0\text{T}})\Upsilon_{k:0}\right].
	% \end{equation}
% These predictions are then compared to the observed frequencies, $n_{i,\vec{\mu}}$. The `likelihood' of $\Upsilon_{k:0}$ subject to the data is given by $\mathcal{L} = \prod_{i,\vec{\mu}} (p_{i,\vec{\mu}})^{n_{i,\vec{\mu}}}$. The cost function of MLE algorithms is then the log-likelihood, i.e.,
% \begin{equation}
	% \label{ML-cost}
	%     f(\Upsilon_{k:0}) = -\ln \mathcal{L} = \sum_{i,\vec{\mu}} -n_{i,\vec{\mu}}\ln p_{i,\vec{\mu}},
	% \end{equation}

	\section{Obtaining Process Tensor Marginals}
\label{app:process-tensors}
We review here the background of process tensors, and detail the procedure to obtain process tensor marginals from the classic shadow data. For a more extensive discussion, see Refs.~\cite{Pollock2018a,Milz2021PRXQ,white2022non}.


\emph{Process tensor framework.--}
A quantum stochastic process describes the non-deterministic dynamics of an open quantum system $\rho^S\in \mathcal{B}(\mathcal{H}_S)$ across a series of times $\mathbf{T}_k=\{t_0,t_1,\cdots,t_k\}$. Specifically, this represents knowledge of the conditional state $\rho_k^S(\mathbf{A}_{k-1:0})$ subject to an arbitrary sequence $\mathbf{A}_{k-1:0}:= \{\mathcal{A}_0, \mathcal{A}_1, \cdots, \mathcal{A}_{k-1}\}$ of control operations at each $t_j$. Note that these controls in full generality constitute non-deterministic maps, such as quantum instruments.
%we consider the situation where a $k$-step process is driven by a sequence $\mathbf{A}_{k-1:0}$ of control operations, each represented mathematically by CP maps: $\mathbf{A}_{k-1:0} := \{\mathcal{A}_0, \mathcal{A}_1, \cdots, \mathcal{A}_{k-1}\}$, after which we obtain a final state $\rho_k(\mathbf{A}_{k-1:0})$ conditioned on this choice of interventions. 
These controlled dynamics have the form:
\begin{equation}\label{eq:multiproc-app}
	\rho_k^S\left(\textbf{A}_{k-1:0}\right) = \text{tr}_E [U_{k:k-1} \, \mathcal{A}_{k-1} \cdots \, U_{1:0} \, \mathcal{A}_{0} (\rho^{SE}_0)],
\end{equation}
where $U_{k:k-1}(\cdot) = u_{k:k-1} (\cdot) u_{k:k-1}^\dag$. Eq.~\eqref{eq:multiproc-app} can be used to define a mapping from past controls $\mathbf{A}_{k-1:0}$ to future states $\rho_k\left(\textbf{A}_{k-1:0}\right)$, which is the process tensor $\mathcal{T}_{k:0}$:
\begin{equation}
	\label{eq:PT}
	\mathcal{T}_{k:0}\left[\mathbf{A}_{k-1:0}\right] = \rho_k^S(\mathbf{A}_{k-1:0}).
\end{equation}
Each intervention $\mathcal{A}_j$ has a Choi representation $\hat{\mathcal{A}}_j$ via the Choi-Jamiolkowski isomorphism (CJI), given by its action on one half of a maximally entangled state $\ket{\Phi^+} = \sum_{i=1}^d\ket{ii}$:
\begin{equation}
	\label{eq:channel-choi}
	\hat{\mathcal{A}}_j = (\mathcal{A}\otimes \mathcal{I})\left[|\Phi^+\rangle\!\langle \Phi^+|\right] = \sum_{i,j=1}^d\mathcal{A}[|i\rangle\!\langle j|]\otimes |i\rangle\!\langle j|.
\end{equation}
The two subsystems of this state can be seen as `input' and `output' spaces: $\hat{\mathcal{A}}\in \mathcal{B}(\mathcal{H}_{\mathfrak{o}})\otimes \mathcal{B}(\mathcal{H}_{\mathfrak{i}})$, since the output state under the action of the map is given on the left space after projecting some state onto the right subsystem. That is, $\mathcal{A}[\sigma] = \text{Tr}_{\mathfrak{i}}\left[(\mathbb{I}_{\mathfrak{o}}\otimes \sigma^{\text{T}})\hat{\mathcal{A}}\right]$.

Through a generalisation of the CJI, process tensors may be represented as a $2k+1$-partite quantum state, $\Upsilon_{k:0}$. Equation~\eqref{eq:channel-choi} is generalised by swapping in one half of a fresh maximally entangled state at each time. This state then predicts multi-time probabilities in accordance with Equation~\eqref{eq:multiproc-app}. That is, when the final state $\rho_k^S(\mathbf{A}_{k-1:0})$ is measured with a POVM $\{\Pi_k\}$, the observed probabilities for each effect is given by
\begin{equation}
	\label{eq:PT-vector}
	p_k^S(\mathbf{A}_{k-1:0})= \text{Tr}  \left[\Upsilon_{k:0}\left(\Pi_k\otimes \hat{\mathcal{A}}_{k-1}\otimes \cdots \otimes  \hat{\mathcal{A}}_0\right)^\text{T}\right].
\end{equation}
Thus, sequences of CP maps constitute observables on the process tensor. If a process output is measured when conditioned on an informationally complete set of instruments, then Equation~\eqref{eq:PT-vector} can be uniquely inverted to reconstruct $\Upsilon_{k:0}$ -- although in practice when the probabilities are actually noisy frequency estimates, an estimation procedure such as maximum likelihood must be employed to ensure physical conditions are imposed, like positivity of the map and causal direction of the statistics. 


% \begin{equation}
	% \label{PT-vector-est}
	%     p_{i,\vec{\mu}} = \text{Tr}\left[(\Pi_i \otimes  \mathcal{B}_k^{\mu_{k-1}\text{T}}\otimes \cdots \otimes \mathcal{B}_0^{\mu_0\text{T}})\Upsilon_{k:0}\right].
	% \end{equation}



The Choi form of a process tensor is an $2k+1$-partite state with process marginals, $\{\hat{\mathcal{E}}_{k:k-1},\cdots,\hat{\mathcal{E}}_{2:1},\hat{\mathcal{E}}_{1:0},\rho_0\}$. Any correlations between these subsystems constitute non-Markovian correlations due to the external environment. In keeping with our channel Choi state convention, we use the notation $\mathfrak{o}_j$ to denote an output leg of the process at time $t_j$, and $\mathfrak{i}_j$ for the input leg of the process at time $t_{j-1}$. The collection of indices is therefore $\{\mathfrak{o}_k,\mathfrak{i}_k,\cdots,\mathfrak{o}_2,\mathfrak{i}_2,\mathfrak{o}_1,\mathfrak{i}_1,\mathfrak{o}_0\}$. 

Assuming now that we have a process tensor defined on a register $\mathbf{Q}=\{q_1,\cdots,q_N\}$, then we can fine-grain not just in time but also in space. We first note that without loss of informational completeness, each instrument $\hat{\mathcal{A}}_j$ can be factored into local operations $\bigotimes_{i=1}^N\hat{\mathcal{A}}_j^{(q_i)}$. The dynamical maps of the process can also be further marginalised in the same way to obtain $\hat{\mathcal{E}}_{j:j-1}^{(q_i)}$: the average CPTP map taking the $i$th qubit from time $t_{j-1}$ to $t_j$. Although process tensors contain information about all multi-time correlations, for simplicity's (and efficiency's) sake, in this work we consider only two map correlations. Therefore, spacetime correlations can be probed across the following pairs of marginals:

\begin{itemize}
	\item \underline{Purely spatial}: $\hat{\mathcal{E}}_{j:j-1}^{(q_n)}$ and $\hat{\mathcal{E}}_{j:j-1}^{(q_m)}$,
	\item \underline{Purely temporal}: $\hat{\mathcal{E}}_{j:j-1}^{(q_n)}$ and $\hat{\mathcal{E}}_{l:l-1}^{(q_n)}$,
	\item \underline{Spatiotemporal}: $\hat{\mathcal{E}}_{j:j-1}^{(q_n)}$ and $\hat{\mathcal{E}}_{l:l-1}^{(q_m)}$.
\end{itemize}

Pure spatial correlations constitute either direct crosstalk, or presence of an environmental common cause factor. As we show in the next section, purely temporal marginals constitute genuine bath non-Markovian correlations. And finally, spatiotemporal correlations indicate two qubits coupled to the same non-Markovian bath.

%\section{Pathways proof}
%\label{app:pathways-proof}
\emph{Distinguishing RNM and BNM.--}
Here, we give a short graphical proof for the fact that applying depolarising channels to other qubits in the register at each time eliminates them as a potential non-Markovian source.
In the dilated open quantum evolution picture, a process tensor may be written as the \emph{link product} $\star$ of a series of $SE$ unitaries. 
\begin{equation}
	\label{eq:PT-link}
	\Upsilon_{k:0} = \text{Tr}_{E}\left[\bigstar_{i=1}^{k} \hat{\mathcal{U}}^{(SE)}_{i:i-1} \star \rho_0^{(SE)}\right],
\end{equation}
where $\hat{\mathcal{U}}_{i:i-1}$ is the Choi representation of the $i$th step unitary $U_{i:i-1}$. This lives on $\mathcal{B}(\mathcal{H})_S^{\mathfrak{i}}\otimes\mathcal{B}(\mathcal{H})_E^{\mathfrak{i}}\otimes\mathcal{B}(\mathcal{H})_S^{\mathfrak{o}}\otimes\mathcal{B}(\mathcal{H})_E^{\mathfrak{o}}$. Suppose the environment factorises into two spaces: $\mathcal{H}_E \cong \mathcal{H}_C \otimes \mathcal{H}_B$ -- the controllable qubits and the uncontrollable bath -- then each $\mathcal{U}_{i:i-1}$ has twelve indices: ket and bra for the input and output spaces for each of $S, C, B$. Equation~\eqref{eq:PT-link} can be written more intuitively using the graphical calculus formalism~\cite{wood2011tensor}, as shown at the top of Figure~\ref{fig:PT-link}.



% \begin{equation}
	% \Upsilon_{k:0} = \sum \delta_{k_k^ck_k^b}^{b_k^cb_k^b} \left(\mathcal{U}_{k:k-1}\right)^{k^s_kk^c_kk^b_k}_{b^s_kb^c_kb^b_k} \left(\mathcal{U}_{k-1:k-2}\right)^{b^s_kb^c_kb^b_k}_{k^s_{k-1}k^c_{k-1}k^b_{k-1}}\cdots \left(\mathcal{U}_{1:k0}\right)^{b^s_kb^c_kb^b_k}_{k^s_{k-1}k^c_{k-1}k^b_{k-1}}
	% \end{equation}
\begin{figure}[h!]
	\centering
	\includegraphics[width=\linewidth]{Shadows_Paper/ST_Fig_App.pdf}
	\caption{Graphical depiction of causal testing. At the top, we represent the process tensor in terms of its dilated link product representation. Below, we show how the transformation implements depolarising channels, leaving the process as tensor product structure across $\mathcal{B}(\mathcal{H}_C)$.}
	\label{fig:PT-link}
\end{figure}

Because depolarising channels are a product state over $\mathcal{B}(\mathcal{H}_{\mathfrak{o}})\otimes \mathcal{B}(\mathcal{H}_{\mathfrak{i}})$, they hence implement a causal break.
Note that any choice of instrument for which the Choi state is a product state (for example, a projective measurement and fresh preparation) constitutes a valid causal break, but a depolarising channel is the only one for which the locality of the observable does not grow, and hence can be efficient under the classical shadows procedure.


\emph{Identifying systems with a shared non-Markovian bath.--}
The same logic applies for the observation of correlations between some $\hat{\mathcal{E}}_{j:j-1}^{(q_n)}$ and $\hat{\mathcal{E}}_{l:l-1}^{(q_m)}$. Obtaining these two correlated marginals means that a causal break is applied at the $\mathfrak{o}$ leg of $\hat{\mathcal{E}}_{j:j-1}^{(q_m)}$ and at the $\mathfrak{i}$ leg of $\hat{\mathcal{E}}_{l:l-1}^{(q_n)}$. Hence, this erases any mixing terms between $\mathcal{H}_{q_n}$ and $\mathcal{H}_{q_m}$ in the unitaries. Consequently, non-zero values for the mutual information between these maps must be due to interactions involving $\mathcal{H}_B$ \& $\mathcal{H}_{q_n}$ at the first time step, and then $\mathcal{H}_B$ \& $\mathcal{H}_{q_m}$ at the second second. I.e. the two qubits shared the same bath. 
%However, the estimations are less useful for processes than their spatial counterparts. The reason for this may be understood that observables of a process are also propagators of the state. If we take these to be low-weight, then at many points in time the state is erased (maximally mixed). Thus, for detectable temporal correlations to persist, the $SE$ interactions must be strong and they must be non-unital at the system level. Moreover, the environment must be large so as to wash away the incoherence.

%It is for this reason that we envisage the utility of shadows on processes to be not in learning a many-step process on a single qubit, but instead to consider a smaller process across a whole register of qubits. By selectively erasing spatial correlations, we can instead determine causal pathways to explain non-Markovian dynamical origins. We consider two possible applications of spatiotemporal classical shadows, and supplement with numerical demonstrations.



\emph{Distinguishing between passive crosstalk and bath non-Markovianity.--}
First, we consider certifying when non-Markovian correlations originate via an inaccessible bath, or from neighbouring qubits in the register.
Certifying bath non-Markovianity means estimating $\Upsilon_{k:0}^{(q_i)}$ -- the marginal process tensor for a single qubit. Through the usual procedure of classical shadows, this can be simultaneously performed for all $q_i\in \mathbf{Q}$. The Choi state of the operations on the remainder of the qubits at each time will be $\mathbb{I}/d$, i.e. a maximally depolarising channel. Because this enacts a causal break -- the operation is a product state -- any information travelling from the system into the register cannot persist forwards in time. Hence, a suitable choice for computing the non-Markovianity in $\Upsilon_{k:0}^{(q_i)}$ will be a measure of correlations from an inaccessible bath alone. We formally show this in the appendix. 

We demonstrate this numerically in Figure~\ref{fig:simulated-baths}. Here, we have 15 qubits and one defect quantum system acting as the bath in a two-step process, and then compute $\mathcal{N}(\Upsilon_{2:0}^{q_i})$. The qubits each experience a random nearest-neighbour $ZZ$-coupling crosstalk, and the ones geometrically closest to the defect are Heisenberg-coupled to that system. Figure~\ref{fig:simulated-baths}a shows the standard fare: estimating the process tensor of each qubit and determining its non-Markovianity while the other qubits remain idle. However, the results are not so informative, because they do not distinguish between RNM and BNM effects, and so every qubit experiences temporal correlations. %Meanwhile estimating a multi-qubit process tensor to incorporate any register correlations quickly becomes infeasible.
We show in Figure~\ref{fig:simulated-baths}b the results of a shadow marginal estimation. 
%The effect of employing classical shadows here is to average out instruments on neighbouring qubits to a maximally depolarising channel; this performs a causal break at each time and filters out the possibility of non-Markovian effects from crosstalk. 
We see that, only the qubits which are actually coupled to non-Markovian bath defects have a non-zero $\mathcal{N}(\Upsilon_{2:0}^{(q_i)})$, and we can readily identify them. 
\begin{figure}[H]
	\centering
	\includegraphics[width=0.75\linewidth]{Shadows_Paper/ST_Fig_4.pdf}
	\caption{
		A numerical simulation demonstrating the proposed technique to determine qubits with shared baths. A grid of 14 qubits is simulated with crosstalk effects and two inaccessible non-Markovian defects. \textbf{a} Shadow filtering may be used to find qubits coupled to an inaccessible bath as before
		\textbf{b} By looking at the correlations between map $\hat{\mathcal{E}}_{1:0}^{(q_m)}$ with $\hat{\mathcal{E}}_{2:1}^{(q_n)}$, we can infer which qubits share common baths and the extent to which the defects redistribute quantum information.
		Note, the relationship lines between qubits are not direct crosstalk interactions, but bath-mediated spatiotemporal correlation.}
	\label{fig:cc-relations}
\end{figure}

\emph{Identifying shared baths.--}
A second important scenario we consider is where two qubits are correlated via common cause from a shared bath. For example, this might be experiencing the same stray magnetic field inhomogeneities or through a coupling to a common defect.
This is sometimes referred to as crosstalk, because the joint map $\hat{\mathcal{E}}_{j:j-1}^{(q_1,q_2)}$ does not factor to $\hat{\mathcal{E}}_{j:j-1}^{(q_1)}\otimes \hat{\mathcal{E}}_{j:j-1}^{(q_2)}$~\cite{Sarovar2020detectingcrosstalk}. However, we consider this a coarse description because neither system acts as a direct cause for each other's dynamics. Instead, they are subject to spatiotemporal correlations as mediated by the same non-Markovian bath -- i.e. the bath is the common cause for the shared correlations. The key, therefore, is to measure the relationship between the maps $\hat{\mathcal{E}}_{j:j-1}^{(q_1)}$ and $\hat{\mathcal{E}}_{j+1:j}^{(q_2)}$.

We demonstrate this numerically in Figure~\ref{fig:cc-relations}. We have a similar setup to before, except this time with two bath defects. Performing a shadow filtering (Figure~\ref{fig:cc-relations}a) again reveals which qubits are coupled to the defects. However, in Figure~\ref{fig:cc-relations}b, we look at the spacetime marginals estimated from the shadow data. This fine-grained data indicates which qubits are commonly coupled to bath defects, versus independently coupled. The arrows from qubit $q_i$ to qubit $q_j$ indicate the QMI in the process with marginals $\hat{\mathcal{E}}_{2:1}^{(q_j)}\otimes \Upsilon_{1:0}^{(q_i)}$.
The erasure of $q_j$ in the first step and $q_i$ in the second step eliminates the possibility of direct-cause correlations between the two qubits, leaving only the possibility of common-cause. In other words, non-zero values are a measure of non-Markovian correlations distributed by a shared bath between two qubits. This generates a more informative view of the interplay between qubits and their environment, breaking down the extent to which different systems share temporal correlations and which are fully independent from one another. %and could feed, for example, into more sophisticated models of error correction decoders.


\section{Discussion}
We have introduced a scalable and conceptually simple method to distinguish between non-Markovian dynamics generated by nearby qubits in a quantum device, and those from an inaccessible bath. 
This contributes to the growing zoo of quantum characterisation, verification, and validation techniques, and yet satisfies a unique niche. Geometrically isolating non-Markovian sources across a device can inform various facets of the development process: the signals can warrant further investigation and inform the fabrication process; they can flag qubits to be given extra control attention; and they can be used in error-finding mechanisms for error-correction decoders.

This also extends the capabilities of the randomised measurement toolbox in the multi-time and multi-qubit domain. Despite the limitations of classical shadows for quantum stochastic processes, we have identified an important use case in efficient casual testing.
We have introduced this in full generality with respect to PTT, however the techniques are generic: the only important point is that causal breaks are applied to neighbouring qubits between each steps. The same principles will broadly apply to other approaches to learning non-Markovian dynamics~\cite{PhysRevLett.124.140502,PhysRevLett.112.110401,nielsen-gst,PRXQuantum.2.040351}.







==> FrontBackMatter/Bibliography.tex <==
% Bibliography
\label{app:bibliography} % Reference the bibliography elsewhere with \autoref{app:bibliography}

\manualmark % Work-around to have small caps also here in the headline
\markboth{\spacedlowsmallcaps{\bibname}}{\spacedlowsmallcaps{\bibname}} % Work-around to have small caps also
%\phantomsection
\refstepcounter{dummy}

\addtocontents{toc}{\protect\vspace{\beforebibskip}} % Place the bibliography slightly below the rest of the document content in the table of contents
\addcontentsline{toc}{chapter}{\tocEntry{\bibname}}

% \printbibliography
\include{main.bbl}


==> FrontBackMatter/Colophon.tex <==
% Colophon (a brief description of publication or production notes relevant to the edition)

\pagestyle{empty}

\hfill

\vfill

\pdfbookmark[0]{Colophon}{colophon}

\section*{Colophon}

This document was typeset using the typographical look-and-feel \texttt{classicthesis} developed by Andr\'e Miede. The style was inspired by Robert Bringhurst's seminal book on typography ``\emph{The Elements of Typographic Style}''. \texttt{classicthesis} is available for both \LaTeX\ and \mLyX: 

\begin{center}
\url{https://bitbucket.org/amiede/classicthesis/}
\end{center}

\noindent Happy users of \texttt{classicthesis} usually send a real postcard to the author, a collection of postcards received so far is featured here: 

\begin{center}
\url{http://postcards.miede.de/}
\end{center}
 
\bigskip

\noindent\finalVersionString

==> FrontBackMatter/Preamble.tex <==
\chapter*{Preamble}

\noindent Some explanation of how to read the thesis
\begin{itemize}
	\item Structure (kind of)
	\item Explanation of the chapter introductions etc.
	\item Maybe some overview of the graphical calculus explanations? Will need to find a home for that
\end{itemize}



In matters arising with respect to the structure of the thesis, \textit{I}, the author, will attempt to be as clear as possible about the approach. This is in order to make the experience as clear as possible for \textit{You}, the reader.
With respect to the science, \textit{We}, author and reader, will traverse this exposition together.
